A Context-Contrastive Inference Approach To Partial Diacritization

Diacritization plays a pivotal role in improving readability and disambiguating the meaning of Arabic texts. Efforts have so far focused on marking every eligible character (Full Diacritization). Comparatively overlooked, Partial Diacritzation (PD) is the selection of a subset of characters to be marked to aid comprehension where needed. Research has indicated that excessive diacritic marks can hinder skilled readers -- reducing reading speed and accuracy. We conduct a behavioral experiment and show that partially marked text is often easier to read than fully marked text, and sometimes easier than plain text. In this light, we introduce Context-Contrastive Partial Diacritization (CCPD) -- a novel approach to PD which integrates seamlessly with existing Arabic diacritization systems. CCPD processes each word twice, once with context and once without, and diacritizes only the characters with disparities between the two inferences. Further, we introduce novel indicators for measuring partial diacritization quality, essential for establishing this as a machine learning task. Lastly, we introduce TD2, a Transformer-variant of an established model which offers a markedly different performance profile on our proposed indicators compared to all other known systems.

==> tables/partial-dd-results.tex <==
\begin{table*}[ht]
\centering
% \begin{tabular}{cc@{\hskip 0.5em}|@{\hskip 0.5em}rrrr}
\begin{tabular}{ccrrrr}
    \toprule
        \bf Dataset & \bf System
        % & \multicolumn{1}{c}{\thead{SR}} & \multicolumn{1}{c}{\thead{PDER}}
        % & \multicolumn{1}{c}{\thead{GE}} & \multicolumn{1}{c}{\thead{TEE}} \\
        & \multicolumn{1}{c}{\bf Selectivity}  & \multicolumn{1}{c}{\bf Partial DER}
        & \multicolumn{1}{c}{\bf Guessability} & \multicolumn{1}{c}{\bf Total DER} \\
    \midrule
        \multicolumn{2}{c}{Reference Range}
            & $13\% \pm 8\%$
        % & \multicolumn{3}{c}{$[0, 100]$: Lower is better}
        & \multicolumn{3}{c}{$100 .. 0$ : Lower is better}
    \\
    \midrule
        \multirow{4}{*}{\dataset{Tashkeela}}
            & \citealp{shakkala}
                                &  6.7\% & 17.9\% &  1.7\% &  2.8\% \\
            & \citealp{fadel-etal-2019-neural}
                                &  8.9\% &  7.8\% &  1.0\% &  1.6\% \\
        % \cmidrule[0.01pt]{2-6}
            & \citealp{alkhamissi-etal-2020-deep}
                                &  6.5\% & 11.2\% &  1.1\% &  1.8\% \\
            & \bf\modelTD{}     & 24.6\% &  5.5\% &  1.4\% &  2.4\% \\
    \midrule
        \multirow{4}{*}{\dataset{Ashaar}}
            & \citealp{shakkala}
                                &  9.3\% & 49.5\% & 17.0\% & 20.1\% \\
            & \citealp{fadel-etal-2019-neural}
                                & xx.x\% & xx.x\% & xx.x\% & xx.x\% \\
        % \cmidrule{2-6}
            & \citealp{alkhamissi-etal-2020-deep}
                                & 11.2\% & 47.3\% & 19.9\% & 23.0\% \\
            & \bf\modelTD{}     & 28.0\% & 26.0\% & 11.5\% & 15.6\% \\
    \bottomrule
\end{tabular}
\caption{Partial Diacritics Results by the metrics outlined in \Secref{sec:new-metrics}. \textbf{SR} is Selection Ratio, \textbf{PDER} is Partial Diacritic Error Rate, \textbf{GE} is Guessability Error, and \textbf{TEE} is Total Error Rate. \modelname{Shakkala} is due to \citet{shakkala}, and \modelname{Shakkelha} is due to \citet{fadel-etal-2019-neural}.
}
\label{table:test_results}
\end{table*}
% \todo{Add remark on range interpretation of the each metric (lower is better for all except SR).}
